SummaryMixing: A Linear-Complexity Alternative to Self-Attention for Speech Recognition and Understanding

Modern speech processing systems rely on self-attention. Unfortunately, token mixing with self-attention takes quadratic time in the length of the speech utterance, slowing down inference and training and increasing memory consumption. Cheaper alternatives to self-attention for ASR have been developed, but they fail to consistently reach the same level of accuracy. This paper, therefore, proposes a novel linear-time alternative to self-attention. It summarises an utterance with the mean over vectors for all time steps. This single summary is then combined with time-specific information. We call this method "SummaryMixing". Introducing SummaryMixing in state-of-the-art ASR models makes it feasible to preserve or exceed previous speech recognition performance while making training and inference up to 28% faster and reducing memory use by half.

==> resources/rtf_figures.tex <==

\begin{figure}[!h]
\begin{center}
\hfill
\includegraphics{figs/resources/decoding_rtf}
\hspace*{1cm}
\includegraphics{figs/resources/decoding_vram}

\caption{ Real Time Factor (left) and peak VRAM consumption (right) obtained with CTC-only greedy batch-decoding (batch size of 16) on audio files of different lengths originating from Librispeech \textit{test-clean} after full-training. Each measurement is an average of 2,500 sentences decoding of the given length. The quadratic-time complexity of the Branchformer impacts the RTF of the decoding process for long sentences while all the other models exhibit an improvement in RTF over long sentences. This is particularly visible for the different Sumformers.   } \label{fig:curves}
\end{center}
\end{figure}


==> sections/background.tex <==
\section{Background and Motivations}
\label{sec:background}

Current SOTA speech recognizers including the Conformer \cite{gulati2020conformer} or the Branchformer \cite{kim2023branchformer,peng2022branchformer} all rely on MHSA. In practice, MHSA is expected to capture a robust global context by modeling relations between pairs of tokens, i.e. speech frames. Then, it is combined with the local filtering capabilities of convolutional networks to benefit from the best of both worlds. The conformer sequentially stacks MHSA with CNN, while the Branchformer proposes to perform both concurrently and then merges the obtained representations. Nevertheless, both architectures rely on global and local context learning.

The first issue of MHSA is its complexity. Indeed, and as it must compute attention weights between all pairs of tokens, its time complexity grows quadratically with the input sequence length e.g. 25 to 100 vectors per second of the speech signal. This issue represents a very active research direction and most lines of work attempt at retaining the modeling capabilities of self-attention while lowering its complexity. Examples include low-rank approximation \cite{tay2022efficient}, linearization \cite{wang2020self} or sparsification \cite{child2019generating}. These methods, however, may imply complex modifications or specific hardware to achieve a speed-up and usually come with a slight degradation in the final performance. This work aims both at speeding up training and inference to increase the adoption of SOTA ASR systems in a wider range of devices and at retaining the remarkable accuracy of MHSA-equipped systems.

Alongside this complexity issue, a recent trend of research calls into question the usefulness of using MHSA to capture the global context necessary to perform speech recognition. Indeed, a few works have demonstrated that once trained, self-attention layers used for ASR end up having attention weights distributed evenly. This has been observed in particular with the Branchformer architecture \cite{peng2022branchformer} and in the upper layer of the Conformer model \cite{shim2022understanding}. Hence we can hypothesize that the capability of MHSA to capture fine-grained and pair-wise global relationships may be unnecessarily costly for ASR systems as a simpler global context may be sufficient.\This work specifically aims at demonstrating that a simpler, i.e. easier to define and cheaper to compute, form of global context is sufficient to achieve SOTA performance in ASR.

MLP Mixer \cite{tolstikhin-2021-mlp} was the first to show that token mixing can also be achieved from outside the framework of attention, opening up considerably novel opportunities for speed and resource consumption improvements. In particular, MLP Mixer learns a fixed-size MLP to perform token mixing throughout time hence achieving competitive performance across a wide range of domains with linear time complexity \cite{choe2022pointmixer}. Unfortunately, speech tasks commonly have variable-length sequences and existing extensions of MLP Mixer to this modality only propose to rely on chunked input vectors \cite{sakuma2022mlp} or achieve sub-optimal performance \cite{sakuma2021mlp}. This article shows that the concept of token mixing originating from MLP Mixer can be generalized with a simpler notation and implementation, and adapted to variable input sequence lengths while retaining MHSA performance.

==> sections/discussion.tex <==
\subsection{Valuable Properties and Limitations}

SummaryMixing emerged at the crossroads of two lines of thought: (a) MHSA seems to be irrelevant for the encoder part of modern speech recognizers; and (b) MLP Mixer could be generalized to a simpler and more powerful definition of a linear alternative to MHSA for variable length sequences such as speech recognition and understanding. The resulting architecture was not expected to drastically outperform MHSA, but instead, to bridge the gap between linear non-attentional encoders and state-of-the-art MHSA encoders. It appears clearly from the conducted experiments that the two initial hypotheses are valid. Indeed, the difference in WER between an MHSA plus CNN and a CNN Only Branchformer is not large, proving that MHSA could be replaced with a simpler global context summarization technique. Then, SummaryMixing outperformed MHSA in all experiments for speech recognition and understanding while remaining much faster and cheaper at training, inference, and decoding resulting in a potentially larger deployment of speech systems in more accessible hardware. 

% A natural extension of the Sumformer would be, however, Transducer architectures for speech recognition. Indeed, by design, Transducers incorporate an implicit language modeling component that helps lifting the need for extended global context from the encoder. Transducers also are well known for significant costs associated with training, and could therefore benefit from the introduction of the Sumformer. They also represent a popular architecture for online or streaming speech recognition. In its current definition, the Sumformer is not compatible with streaming ASR. Nevertheless, due to the simplicity of the formulation of the Summary Mixing that can be understood as a gated average of the global context, one may naturally extend the Sumformer to an incremental Sumformer updating its global context while new frames of speech are coming. Since the focus of this work was to introduce the principal motivations and foundations of the Sumformer, we leave specialized ASR systems, such as streaming networks, for future work. 

Finally, we wish to highlight that the SummaryMixing mechanism structurally can not model complex global dependencies between tokens as MHSA does, and this is a feature rather than a problem when the MHSA pair-wise interaction is not necessary, as in speech recognition. {This is validated by the results observed without attentional decoders, i.e. CTC only training and decoding, for ASR as the SummaryMixing Conformer obtained the same performance as the self-attention-based equivalent, proving that self-attention may not be necessary to reach state-of-the-art performance.}



==> sections/introduction.tex <==
\section{Introduction}


Automatic speech recognition has greatly benefited from deep learning, reaching unprecedented levels of accuracy and enabling a number of successful products to support real-life use cases \citep{nassif2019speech}. 
ASR systems have followed the general trend in deep learning and increased steadily both in model size and complexity to push recognition accuracies. 
Modern industry-scale ASR models often contain hundreds of millions or even billions of neural parameters \citep{radford2022robust}.
However, at the same time, the demand for resource-efficient deployment of on-device ASR models is gaining in popularity as more and more smart devices are pervading our everyday lives, not only for efficient inference but also for on-device training \citep{arasteh2016iot}.

%However, another growing trend is advocating for the deployment or even training of ASR systems on constrained devices. The latter use cases answer a very particular market space as more and more smart devices surround us \citep{arasteh2016iot} raising very practical questions about resource efficiency.

At the core of current state-of-the-art (SOTA) ASR systems are the multi-head self-attention cells \citep{vaswani2017attention}, an elegant and powerful way of generating fine-grained global interactions between pairs of tokens, i.e., frames in the context of speech signals, also referred to as token mixing. 
MHSA is responsible for learning both interactions between frames originating from the speech signal, which has helped reach SOTA performance in most ASR paradigms, including Transducers \citep{gulati2020conformer}, encoder-decoder and encoder-only systems \citep{peng2022branchformer,baevski2020wav2vec}. 
It also applies to streaming \citep{li2021better} or offline speech recognizers \citep{kim2023branchformer}.
Despite its success, MHSA is costly to use both during training and inference, especially for ASR systems dealing with long utterances due to the requirement of computing attention weights between all pairs of tokens, i.e., the time complexity grows quadratically with the input sequence length.
%Nevertheless, MHSA may be costly to use at training time, but also during inference, for ASR systems dealing with long utterances. 
 
%e.g. 25 to 100 vectors per second of the speech signal. 
Thus, developing efficient attention mechanisms has been an active area of research and a number of attempts have been made to address the problem. Successful examples include low-rank approximation \citep{tay2022efficient}, linearization \citep{wang2020self} or sparsification \citep{child2019generating}.
%This issue represents a very active research direction and most lines of work attempt at retaining the modeling capabilities of self-attention while lowering its complexity. Examples include low-rank approximation \citep{tay2022efficient}, linearization \citep{wang2020self} or sparsification \citep{child2019generating}. 
These methods often approximate the pair-wise attention scores and may imply complex modifications or specific hardware capabilities to achieve a speed-up. Approximations of attention usually result in a slight degradation in performance. In this work, we focus on novel linear complexity alternatives to MHSA that are not approximating pair-wise scores as they appear to be irrelevant for ASR.

Indeed, recent works in speech recognition pointed out that expansive MHSA operations may not be necessary. 
For example, \citet{zhang2021usefulness} first show that the upper encoder layers in trained Transformer-based ASR models behave like feed-forward layers, which is also verified in \citet{shim2022understanding} for SOTA Conformer models.
%Previous works also suggest in the current SOTA offline speech recognition models, Conformer \citep{gulati2020conformer} and Branchformer \citep{peng2022branchformer}, the quadratic MHSA operation could be redundant.
%\citet{shim2022understanding} show for trained upper Conformer layers the MHSA %also acts like feed-forward layers. 
Furthermore, \citet{peng2022branchformer} demonstrate that the attention matrices of trained Branchformer models tend to have diagonality scores \citep{zhang2021usefulness} near 0.5, which indicates that the attention weights are distributed almost uniformly and a simple average could achieve a similar token mixing.
Therefore, with certain architectures, we hypothesize that MHSA will not bring enough value to the ASR system to justify its significantly higher computing and memory costs. 
The MLP Mixer \citep{tolstikhin-2021-mlp} was the first to show that token mixing can also be achieved from outside the framework of attention, opening up considerably novel opportunities for speed and resource consumption improvements.
%{\color{blue} In this work, we thus search for alternatives to speed up training and inference time of SOTA ASR systems. An efficient yet accurate ASR system will allow for its adoption to a wider range of resource-limited devices.}
%Hence, alternatives to MHSA should be investigated, and this work specifically aims both at speeding up training and inference to increase the adoption of SOTA ASR systems in a wider range of devices and at retaining the remarkable accuracy of MHSA-equipped systems.

MLP Mixer learns a fixed-size MLP to perform token mixing throughout time and achieves competitive performance across a wide range of domains with linear time complexity \citep{choe2022pointmixer}. 
Unfortunately, speech tasks commonly have variable-length sequences and existing extensions of the MLP Mixer to this modality only propose to rely on chunked and fixed-length input vectors and achieve sub-optimal performance \citep{sakuma2021mlp}. 
In this article, we show that the concept of global context with linear complexity from MLP Mixer can be formally generalized to deal with variable-length sequences, such as for speech recognition. We denote this new class of methods as ``Summary Mixing''. We also show that HyperMixer \citep{mai2022hypermixer}, a first attempt at extending MLP Mixer to varying time dimensions in the input space, is in fact a particular case of Summary Mixing leading to an unnecessary slower training time compared to Summary Mixing. The main contributions of this work are three-fold. First, it formally generalizes the concept of MLP Mixer to Summary Mixing for ASR (Section \ref{subsec:summarymixing}). Then it adapts a SOTA offline ASR model to employ Summary Mixing leading to the Sumformer architecture exhibiting linear time complexity while retaining SOTA performance (Section \ref{subsec:sumformer}). Finally, it releases the code within the widely-adopted SpeechBrain toolkit to facilitate reproducibility and encourage further study\footnote{The source code is available at \Url{https://github.com/SamsungLabs/SummaryMixing}}.

The conducted efficiency measurements (Section \ref{subsec:efficiency_analysis}), as well as experiments on two different ASR datasets (Section \ref{subsec:exps_ctcatt}), show that the Sumformer achieves a training time reduction of up to 27\%, an inference time gain of 1.4 times while halving the memory consumption and retaining SOTA ASR performance compared to a Branchformer equipped with MHSA. 


